Learning the Truth From Only One Side of the Story

Learning under one-sided feedback (i.e., where we only observe the labels for examples we predicted positively on) is a fundamental problem in machine learning -- applications include lending and recommendation systems. Despite this, there has been surprisingly little progress made in ways to mitigate the effects of the sampling bias that arises. We focus on generalized linear models and show that without adjusting for this sampling bias, the model may converge suboptimally or even fail to converge to the optimal solution. We propose an adaptive approach that comes with theoretical guarantees and show that it outperforms several existing methods empirically. Our method leverages variance estimation techniques to efficiently learn under uncertainty, offering a more principled alternative compared to existing approaches.

==> conclusion.tex <==
%\section{Conclusion}
%{\large \bf Conclusion}


%and there has been little work done in methods to alleviate its effects. are sub-optimal, showing that these  are not the best choices oftentimes default approaches
% We used a popular linear bandit framework \cite{glm_bandit} and defined a new notion of regret for the one-sided learner. We then presented an adaptive UCB-based method which has both theoretical guarantees and strong empirical performance, outperforming a number of baselines. We believe this work can have potential widespread impact as one-sided feedback is ubiquitous in machine learning and our presented approach can be adapted to more general model classes such as neural networks, which is a direction of future research.

==> old_intro.tex <==



%In this paper we think of the decision maker as a service provider that is interested in lending its services (henceforth referred to as accepting) to as many individuals that request it as possible, as long as doing so does not incur any substantial loss. The service provider decides to which individuals to accept based on a model of the customer's behavior built and trained on the data available to it. The service provider and its customers interact in a sequential manner, where the only data available for the service provider to update its predictive model comes from customers that have been accepted by the service provider's model in the past. 


 %Throughout the fairness literature, the focus has mainly been to devise methods to correct what we call systemic discriminatory biases, resulting of societal and historical interactions between different protected groups. There is a vast literature on the right methodologies to correct for these biases, most often focused on the concept of affirmative action. These have given rise to popular fairness criteria which seek to correct for these systemic biases by attempting to ensure prediction quotas are achieved within each of several protected groups. 


%In this work we depart from studying systemic discrimination and

%In this work we study what we call \textit{emergent discrimination}, that which results, often as an unintentional consequence of using predictive models to make decisions on a population of individuals. We show that a naive use, training and deployment of a predictive model can have unintended and harmful consequences. ... \textcolor{red}{Cite Juanky's paper?. } 

%Consider a simplified example of predicting loan repayment. A bank might estimate that a loan applicant has an elevated risk of default, and will act on it by denying her a loan. The bank, unable to learn about this applicant's true loan repayment behavior, may also deny loans to similar individuals. On the flip side, individuals that may have been given a loan by the bank and repaid it, can cause the bank to over emphasize giving out loans only to similar individuals, to the detriment of other potentially credit worthy customers, thus inadvertently entering into a discriminatory cycle. Putting it in other words if the bank's predictive model is carelessly updated and used it may end up converging to a model that denies loans to customers that would have paid them, and / or it may consistently discriminate against some types of customers while it reaches convergence. 









%Among other things, we show that widely disparate treatment of individuals may emerge as a result of these dynamic interactions between a learner that is trying to fit a model while at the same time using these predictions to decide which datapoints outcomes to observe and incorporate into model training. 

%\textcolor{red}{Mention how this is related to Max' paper and say that we depart from their treatment as we do not consider group fairness ....?}



%\textcolor{red}{If different populations have different statistical properties then satisfying group fairness will be at odds with accurate classification. Instead of assuming access to a metric between individuals, .. we adopt the fairness notion in \cite{} . }

%\textcolor{red}{We do not consider the issue of fairness but certainly our results could be framed through the lenses of fairness. In this case, we are using the fairness notion of Roth and Kearnes, of utility maximizing decision rules.  }


%\textcolor{red}{We instead follow the reasoning of ... w. }





%The fairness concept we introduce to deal with  emergent discriminatory behavior is that of model truthfulness. That is, a learner should ``accept" all datapoints that would result in a positive utility, and reject the remainder. For example a bank should give out loans to all individuals that will repay those loans, and should deny loans to those individuals that will not be able to repay. For the purpose of this work, any other considerations will be deemed moot.



%We are mostly concerned with the dynamical interaction between a learner and its decisions, and how these will affect the distribution of the data used by the learner to update its model, and not with the static predictions a learner may be able to make if it had a priori access to a large amount of unbiased data. %For this reason, we are particularly interested in devising procedures that can ensure a learner , 

% \textcolor{red}{We are interested in understanding }

% We recognize two competing components of the interaction we study:
% \begin{enumerate}
%     \item Learning: The learner's objective is to learn about points that have not been observed yet. Generous acceptance rates can harm the learner's short term utility.
%     \item Acting:  The learner's goal is to make accurate decisions in order to minimize losses and maximize gains. Fixating on only accepting datapoints whose predictions are favourable for the learner, will cause the learner's model to be unbalanced thus causing discriminatory decisions.  
% \end{enumerate}

% We strive for a balanced interaction between these two: a learner that strives to learn and act truthfully, while maximizing its utility. 


%\textbf{Acting truthfully is in the interest of the learner}
%\textbf{A truthful decision rule is utility maximizing.}


%We are not looking for prescriptions to fix systemic discriminatory biases by altering model predictions to fit quotas, but we are aiming to act truthfully. 

%In particular, even without defining explicitly what a protected group is, it is possible to show that careless training of a predictive model can result in a classifier that ... discriminates against a section of the population.   



%Throughout the fairness literature, the focus has mainly been to devise methods to correct "extrinsic" biases, those  resulting of societal dynamics that have caused discriminatory behaviors towards protected groups. There is a vast literature on the right methodologies to correct for these biases, most often focused on the concept of affirmative action. These have given rise to population fairness criteria which seek to correct for these "extrinsic" biases by altering model predictions to ensure prediction quotas are achieved within each of the protected groups. 

%In this paper we focus on a very different yet complementary problem. We instead shed light on what we term "intrinsic" biases, emerging not as a result of societal processes, but from utilizing a model to make decisions that may affect what data is used to train it. Our work revolves around the online formulation of this issue: If the data we are to use in order to train a model is arriving at the same time as the model is being used to make decisions on said datapoints, meaning their labels may not be available unless the model has accepted them, will unintended biases arise, and if so how should we correct for these. In short we ask the question, how do we correct for model training when the training data is biased not as a result of an extrinsic mechanism, but because it is produced by the model we are trying to train. 

%The two main goals of this work are: show intrinsic biases can arise if careless data collection is coupled with model deployment, and to introduce algorithms to mitigate for these biases. We are not looking to propose ways to correct for what we have termed "extrinsic" biases. Instead we argue for a more basic property of a data collection and model mechanism, which we term truthfulness. A learned model is fair if it treats people truthfully within its model class. 

%We study the sequential decision process e... and the quality of the predictions and their impact on protected groups. 




\subsection{Setup}



We consider a learner tasked with making predictions over data points $Z=(X,Y)$ drawn i.i.d. from a distribution $\mathcal{D}$ and supported on $\mathcal{X} \times \mathcal{Y} $ with $\mathcal{X} \subseteq \mathbb{R}^{d}$ and $\mathcal{Y} \subseteq \mathbb{R}$.  The learner makes use of a predictive model $m$ in a class of predictive models $\mathcal{M}$ with $m : \mathcal{X} \rightarrow \mathcal{Y}$ and gets to observe the labels $Y$ only\footnote{Although we only consider threshold decision rules with a fixed known threshold $c$, we note this definition is not as restrictive as it seems as more complex decision rules can be incorporated into our framework by choosing more complex model classes $\mathcal{M}$ . \aldo{Perhaps explain this better}} when the value $m(X) \geq c$ for some known threshold $c$. 

The learner's objective is to find a predictive model $m^*$ maximizing its expected utility as given by a utility function $U:\mathcal{Y} \rightarrow \mathbb{R}$ and a threshold decision rule \footnote{We define a decision rule as a procedure that takes a model $m$ and a datapoint $X$ and produces an indicator variable encoding whether to observe label $Y$ or not. }: \qijia{Could probably use a bit more elaboration on what utility entails here - but I'm guessing you'll cover that in the previous section.}

\begin{equation}\label{equation::learning_objective}
    m^* = \arg\max_{m \in \mathcal{M}} \mathbb{E}_{(X, Y) \sim \mathcal{D}} \left[  U(Y)\mathbf{1}( m(X) \geq c  )\right]. 
\end{equation}
Where $\mathbf{1}(\cdot)$ defines the indicator function. \qijia{Ask Aldo about $\mathbb{E}[\cdot]$.} Although the objective in \eqref{equation::learning_objective} can be thought of as a form of supervised learning loss, we are not only concerned with finding $m^*$, but how acting on models encountered while learning and trained on data dependent on past decisions can lead to numerous pitfalls \aldo{I would like this last sentence to be there but rewritten}. 














\textcolor{red}{The goal of risk minimization is to find a decision rule, specified by model parameters $\theta$, that performs well on a fixed joint distribution over covariates $X$ and an outcome $Y$. }




\subsection{Non-Discriminatory Models and Learning.}


\aldo{Add some philosophy. Why do we call utility maximizing rules non-discriminatory.}

\begin{definition}
We say a model is \emph{non-discriminatory} for a model class $\mathcal{M}$ and utility function $U: \mathcal{Y} \rightarrow \mathbb{R}$ if it is utility maximizing. 
\end{definition}








Next we define non discriminatory learning. \textcolor{red}{segway}

\paragraph{Learning procedures.} A learner is tasked with making predictions during rounds $t=1, \cdots, T$. In each round it is presented with a set of $K$ covariates $\{X_t^{(i)}\}_{i=1}^K$. We allow for \textbf{improper} learning, \textcolor{red}{Insert citation} that is the model $m_t$ used by the learner at time $t$ may be drawn from a model class $\mathcal{M}_t \supseteq \mathcal{M}$. \textcolor{red}{Why??... this is a common assumption .. in cite cite cite and we would be in trouble otherwise?}. Making use of the threshold decision rule $\mathbf{1}(m_t(X) \geq c)$, the learner observes the responses $\{Y_t^{(i)}\}_{i \in S_t}$ of only a subset of covariates $S_t \subseteq \{1, \cdots, K\}$. \textcolor{red}{The learner makes use of this feedback to update its model $m_{t+1}$. } We denote a learning procedure by its sequence of predictive models $\{ m_t \}_{t=1}^T$. 

We are concerned with devising learning procedures that are able to converge to a non-discriminative model:

 \begin{definition}[Endpoint Non-discrimination]
 We say a learning procedure is \emph{endpoint non-discriminatory} if it converges to a model achieving a utility at least as large as that of a non-discriminatory model.
 \end{definition}

Let $\mathbf{Z}_t = \cup_{l = 1 }^t \{(X_l^{i}, Y_l^{(i)} \}_{i \in S_l}$ be the labeled data the learner has access up to round $t$. $\mathcal{Z}_t$ resulted from the complex interaction between the learner, its model update rule and the data. The simplest \aldo{very charged word} learning procedure we study is what we call Greedy learning \aldo{Cite something? Why should we consider this procedure?} :
 
 \begin{definition}[Greedy learning]
 We say that a learner is using a greedy learning procedure if:
 
 \begin{equation*}
     m_{t+1} = \arg\min_{m \in \mathcal{M}} \frac{1}{|\mathbf{Z}_t |} \left(  \sum_{l=1}^{t} \sum_{i \in S_l} \ell( X_l^{(i)}, m(X_l^{(i)}), Y_l^{(i)}) \right)
 \end{equation*}
 For some loss\footnote{\aldo{ Notice the difference between $\ell$ and $U$ and even $U \mathbf{1}( )$. }} function $\ell: \mathcal{X} \times \mathcal{Y} \times \mathcal{Y} \rightarrow \mathbb{R}$. 
 \end{definition}
 
 Although simple and ubiquitously used \aldo{Is it used?}, we show Greedy learning may be discriminatory. In section \aldo{Insert} we show theoretically and experimentally that even for simple linear model classes in both classification and regression the Greedy learner may fail to converge to an endpoint non-discriminatory model.  
 

 
 When each predictive model in $\mathcal{M}$ is parametrized by $\theta \in \Theta \subseteq \mathbb{R}^D$ for some $D \in \mathbb{N}$, the learner may consider taking gradient steps to update its model. The simplest gradient based learning procedure we study is what we call Batch Greedy Learning:
 
 \aldo{If we allow for improper learning of greedy learners can we get non-discriminatory stuff?. Can we get experiments or theory for this?}
 
  \begin{definition}[Batch Greedy learning]
 We say that a learner is using a batch greedy learning procedure if:
 
 \begin{equation*}
     \theta_{t+1} = \theta_t - \eta \frac{1}{|\mathbf{Z}_t |} \left(  \sum_{l=1}^{t} \sum_{i \in S_l} \nabla_\theta \ell(\theta_t,  X_l^{(i)}, Y_l^{(i)}) \right)
 \end{equation*}
 For some loss function $\ell: \Theta \times \mathcal{X} \times \mathcal{Y} \rightarrow \mathbb{R}$. %\qijia{Do you want to put $\theta$ somewhere in the loss?}
 \end{definition}

 
 
 
 
 
 
We focus on the following two scenarios and model classes: 
 


\paragraph{Linear Classification.} In this setup $Y = \{ 0,1\}$ and each  $m \in \mathcal{M}$ corresponds to a $d$-dimensional logistic regression model parametrized by $\theta \in \mathbb{R}^d$ i.e. $m(X) = \frac{ \exp(-\theta^\top X) }{1 + \exp(-\theta^\top X )}$. We define $U(Y) =Y - 0.5 $.  The loss $\ell(\theta, X,  Y)  = -Y\cdot \theta^{\top}X+\log(1+e^{\theta^{\top}X})$ is the standard logistic regression loss. \aldo{There is another important issue here. Are we restricting ourselves to the realizable case? If so, should we define the utility to be $(\theta^*)^\top  X  - 0.5$ as opposed to $(\theta^*)^\top  X - 0.5 + \xi$ where $\xi$ is the noise?} \qijia{I guess it's sort of the notion of pseudo-regret that we are working with here - model doesn't have to be realizable but we compare against $\mathbb{E}[Y|X]$. That seems to be what ppl usually do, no?}
 
 \paragraph{Linear Regression.}  In this case each $m \in \mathcal{M}$ corresponds to a $d$-dimensional linear regression model parametrized by $\theta \in \mathbb{R}^d$ i.e., $m(X) = \theta^\top X$. We define $U(Y) = Y-c$. The loss $\ell(\theta, X, Y) = (\theta^\top X - Y)^2 + \lambda \| \theta \|^2$ with $\lambda \geq 0$ is the standard ridge regression loss.
 

We not only care about desigining procedures that are able to converge to a non-discriminatory predictive model but also on the pathwise effect the learner's decisions may have on the datapoints it encounters. We borrow concepts from online learning to capture a measure of pathwise discrimination. Define the \aldo{(discriminative?)} regret of a learning procedure $\{m_t\}$ as follows:
\begin{equation}
    \mathcal{R}(T ) = \sum_{t=1}^T \sum_{i = 1}^K U(Y_t^{(i)}) \mathbf{1}( m^*(X_t^{(i)}) \geq c ) - \sum_{t=1}^T \sum_{i=1}^K U(Y_t^{(i)}) \mathbf{1}( m_t(X_t^{(i)}) \geq c ). 
\end{equation}
The regret measures how far ...

\begin{definition}[Path Non-discrimination] We say a learning procedure is path non-discriminatory if its expected regret is sublinear:
\begin{equation*}
    \mathcal{R}(T) = \mathcal{O}(T^{\alpha}). 
\end{equation*}
For some $\alpha <1$. \aldo{What is the dependence on $K$?}
\end{definition}

 We make the distinction between endpoint non-discrimination and path non-discrimination to distinctly capture our two goals of achieving non discrimination while learning and after convergence. \aldo{In section [X] we show the greedy learners are path discriminative and show alternatives that mitigate these effects... in both the full minimization and the batch seting. }.
 


\subsection{Emergent discrimination in Greedy learners}

 
Below we give our first result:

\begin{theorem}
 Greedy learning for logistic regression models (or linear regression) models may not yield an endpoint non discriminatory model. 
\end{theorem}
 
 \begin{proof}
 Insert proof.
 \end{proof}
 
 \textcolor{red}{In section (insert reference) we show that in the cases the greedy learner converges to the truthful classifier, it does so at a much slower rate than the (insert the name of the learner we will come up wtih)  }
  \textbf{Greedy learning taking stochastic steps on the accepted datapoints.}

 
\qijia{Should be pushed to a different section.} We show that a greedy learning procedure can result in systematic underadmissions for underrepresented members of the population. In other words, a greedy learning procedure will overly discriminate against members of (a posteriori defined) protected groups. Plainly speaking, early during training a greedy learning procedure will allocate more weight to individual's traits that are strongly correlated with the predicted outcome with the consequence that its data selection mechanism will overly fixate on these traits, thus rejecting individuals that could generate a large utility for the learner, but happen to lie within a wider group that early during training is disfavored by the model. 
 

 
 
 \begin{figure}[hb!]%[H]
  \begin{center}
%    \includegraphics[width=0.40\textwidth]{figures/OLS_simulation_greedy_lower_bound.png}
 %   \includegraphics[width=0.47\textwidth]{figures/logistic_simulation_greedy_lower_bound.png}
    \end{center}
  \caption{Example of when greedy fails to converge to the right solution on discrete 1-dimensional simulated data while our adaptive approach has vanishing regret. {\bf Left}: We use OLS as the learner on the following distribution. $x$ is drawn uniformly on $\{-1, 1\}$ and $P(y=1|x=-1) = 0.6$, $P(y=0|x=-1) = 0.4$ and $P(y=1|x=1) = 1$. If the model learns $(-1, 0)$ before it sees $(-1, 1)$, then it will always have negative predictions for $x = -1$ and thus never observe more instances and learn that it is optimal to predict positively for $x = -1$. Thus with probability $0.4$, the greedy method will not converge to the optimal model. {\bf Right}: We use Logistic Regression as the learner on the following distribution. $x$ is drawn uniformly from $\{-1, 1, 2\}$ and $P(y | x=-1) = 0,  P(y | x=1) = 0.7, P(y | x=2) = 1$. }
	\label{fig:lower_bound}
\end{figure}
 
 \qijia{My attempt at generalizing your example so it (hopefully) looks slightly less contrived ;) Suppose every day we are given two contexts: one is always $e_1\in\mathbb{R}^d$ and the other one is $e_i$ for some $i\in[d]\neq 1$ u.a.r (think of $e_1$ as majority and the other minority). Moreover, the response takes binary values where $\mathbb{P}(y=1|e_1) = 1-\delta_1$ and $\mathbb{P}(y=1|e_i) = 1/2+\delta_i$ for $i\neq 1$ and we care about cutoff at $c=0.5$. After the first step, with probability at least $(1-\delta_1)(1/2-\delta_i)$, we would have the estimate $\hat{\beta}_1 = e_1$, after which none of the $e_i$ from the same group would be observed; and with probability $(1-\delta_1)(1/2-\delta_i)$ we would have $\hat{\beta}_1 = e_1+e_i$ and $\hat{\beta}_t[i]$ would slowly converge to $1/2+\delta_i$ as time progresses, although slow, since on average we observe $e_i$ once in every $d$ time steps. And we can recurse on any one of the rest $d-2$ groups to make probability about non-convergent behavior worse. We can also make response $y$ continuous - just make sure the first example from $e_i$ has response below cutoff $c$, and even if the first one is above $c$, the large variance in the group can still push $\hat{\beta}_t[i]$ below $c$ such that learning halts for group $i$. Morally speaking, I think this example is saying - if we have majority group with slightly higher mean but very concentrated and minority group slightly lower mean but very spread out then it will be bad news for minority if we do greedy (some separation/non-overlapping across groups is also needed). Since we are working with standard basis, this is essentially like MAB if you think about it ... and you just need more samples for estimating the mean to the same confidence level if the variance is large (and therefore incur more regret along the process). This argument will probably go through with near-isometric design as well.}
 

 
 
 
 
 \textcolor{red}{Run this with higher order models, as it may be the case that these ones are even worse in their discriminatory stuff because they are not as rigid. .}

 
 
 \subsection{Online learning}
 
 
 As mentioned in Section \ref{sec::intro} we are interested not only in converging to a truthful model but to act truthfully while doing so. For the purpose of quantifying this goal we introduce the notion of regret:
 
 \begin{equation*}
 \mathcal{R}(T) = \sum_{t=1}^T u(y_t) \mathbbm{1}(m(x) \geq c) - u(y_t)d_t
 \end{equation*}
 
 Where $y_t$ is the (possibly unobserved) signal from the $t-$th individual $x_t$ and $d_t \in \{ 0,1\}$ is the learner's decision of observing it (or not) \qijia{Is $\mathbbm{1}(m(x) \geq c)$ and $d_t$ the same thing?} \aldo{Yes. I was struggling if to define the decision rule to be comparing with a threshold or to make it more general somehow.}. For any decision/learning procedure $\mathcal{R}(T)$ captures its deviation from truthfulness.
 
